Let's Negotiate! A Survey of Negotiation Dialogue Systems

Negotiation is a crucial ability in human communication. Recently, there has been a resurgent research interest in negotiation dialogue systems, whose goal is to create intelligent agents that can assist people in resolving conflicts or reaching agreements. Although there have been many explorations into negotiation dialogue systems, a systematic review of this task has not been performed to date. We aim to fill this gap by investigating recent studies in the field of negotiation dialogue systems, and covering benchmarks, evaluations and methodologies within the literature. We also discuss potential future directions, including multi-modal, multi-party and cross-cultural negotiation scenarios. Our goal is to provide the community with a systematic overview of negotiation dialogue systems and to inspire future research.

==> 11_ethic.tex <==
\section*{Ethical Considerations}



==> 1_introduction.tex <==


\section{Introduction}
\label{section:intro}
% \begin{quote}
%     ``"
%     \qauthor{\textit{}}
% \end{quote}

\epigraph{\textit{``Let us never negotiate out of fear. But let us never fear to negotiate.''}}{\textit{John F. Kennedy}}

%Negotiation is a common strategic communication between two or more people to resolve points of difference, gain an advantage for an individual or collective, or craft outcomes to satisfy various interests~\cite{}. It is pervasive in human daily interaction, which occurs when people communicate to manage conflict or make compromises. An agent that can understand human language and negotiate logically, would significantly benefit human society, from bargaining prices to high-stake political or legal situations. 

Negotiation is one of the crucial abilities in  human communication that involves 
two or more individuals discussing goals and tactics to resolve conflicts, achieve 
mutual benefit, or find mutually acceptable solutions~\cite{fershtman1990importance,bazerman1993negotiating,lewicki2011essentials}. 
It is a common aspect of human interaction, occurring whenever people communicate
in order to manage conflict or reach a compromise. Scientifically, one of the long-term 
goals of dialogue research is to endow intelligent agents with such an ability. The
incorporation of such agents in negotiations could yield significant benefits in many scenarios,
from bargaining prices in everyday trade-in~\cite{he2018decoupling} to high-stakes political
or legal situations~\cite{basave2016study}.

\begin{figure}
    \centering  
    \includegraphics[width=0.49\textwidth]{images/intro.pdf}
    \caption{The negotiation process involves a multi-turn interaction between agent and human. They exchange information about their deals and end up with accepting or declining deals.}
    \label{fig:intro}
\end{figure}

Negotiation dialogue systems~\cite{lewandowska1982meaning,lambert1992modeling,chawla2021casino}\noteIZ{Citation to Chu Carrol and Carberry missing. There should be other works between 1995 and 2021 -- this seems incomplete}
is a research field that aims to build intelligent conversational agents that can automatically
negotiate with a person in natural language, \eg\ CICERO\footnote{\url{https://ai.facebook.com/research/cicero/}} 
from Meta AI. Agents negotiate with humans through multi-turn interactions (Figure~\ref{fig:intro}) 
using \trackIZ{logical reasoning~\cite{sycara2010agent} over  goals~\cite{zhang2020learningbebavior}, 
strategies~\cite{zhou2019augmenting} and psychology factors~\cite{yang2021improving}.}\noteIZ{Is the 
logical reasoning applied to all these?}
A successful negotiation process involves efficient information exchange, 
strategic discussion toward goals, and a closing section.\noteIZ{wouldn't an unsuccessful dialogue gave the same components?}  
% Despite many research work has been proposed in the task, we find a comprehensive survey is missing. In this work, we propose a survey of negotiation dialogue system from benchmarks, methodology, evaluation and future directions. Various benchmarks have been proposed in the recent years, which includes different scenarios, such as bargaining, game, job interview, persuasion. We categorize these datasets based on the strategy type: distributive, such as bargaining, and integrative, such as maximizing outcomes.

Despite the significant amount of research that has been conducted on the task, we are not aware of
a systematic review of the topic. In this work, we aim to fill this gap by reviewing contemporary 
work in the field of negotiation dialogue systems, covering aspects such as benchmarks, evaluation,
methodology and future directions. 
In recent years, various benchmarks have been proposed for negotiation dialogue systems ranging from 
bargaining~\cite{lewis2017deal} and game scenarios~\cite{stac2016discourse} to job 
interviews~\cite{zhou-etal-2019-dynamic} and item exchanges~\cite{chawla2021casino}.\noteIZ{What sort of range is this, and why are benchmarks mentioned here? Move to a more appropriate place} 
Our survey will provide an overview of these benchmarks, and discuss how they have been
used to evaluate the performance of negotiation dialogue systems.


Modeling the negotiation process for conversational agents imposes various challenges. 
Firstly, these agents must be able to reason about and employ various strategies in different 
situations. In addition to strategy modeling, it is also necessary to model the personalities 
\trackIZ{(\eg\ mind, emotion and behaviors)}\noteIZ{This is not personality} of the negotiators. 
Thirdly, an effective policy learning method is advantageous for negotiations. To address these 
challenges, we can categorize existing solutions into three areas: (1)~model users' personalities
to understand negotiator's preferences, (2)~model strategies to enable agents to make reasonable
decisions based on gathered information, and (3)~learning policies to utilize information effectively
in order to optimize results.

In summary, our contributions are three-fold: (1)~we systematically categorize current negotiation 
dialogue benchmarks from a distributive and integrative perspective, with each category based on 
different goal types and tasks; (2)~we categorize typical evaluation methods and current solutions 
into a taxonomy; and (3)~we point out current limitations and promising future research directions.

% Outlines:

% \textbf{Paragraph 1:} broad definition of negotiation in human communication. Highlight its importance of negotiation dialogue systems. briefly introduce the function of negotiation dialogue agents.

% (e.g., Negotiation is a common strategic communication between two or more people to resolve points of difference, gain an advantage for an individual or collective, or craft outcomes to satisfy various interests~\cite{} .)

% \textbf{Paragraph 2:} Highlight the promising research value of negotiation dialogue systems (giving citation). specific definition of the task of negotiation dialogue (using a figure to illustrate if possible).


% \textbf{Paragraph 3:} Introduce the challenges that Negotiation dialogue still faces. using itemsize to list out.


% \textbf{Paragraph 4:} highlight our motivation to propose this survey. introduce the structure of following parts. 

% \textbf{Paragraph 5:} Shortly summarize our contributions.




==> 2_social_impact.tex <==
%\section{Social Impact}
\section{Background}
\lizhen{still thinks it would be a good idea to discuss human limitations in terms of negotiations.}
\subsection{Human Negotiations}
%% Suraj

% concepts of negotiation,
% lay out some foundation for this concept.

% negotiation in real-world

% \subsection{Negotiation in Social Science}

% Introducing the function of negotiation in human communication from the perspective of social science, including psychology, 

% (useful reference: \cite{fershtman1990importance,bazerman1993negotiating,lewicki2011essentials,o2015persuasion})

% Framework:
% (1) Negotiation in human and its function
Humans negotiate everyday in their daily routines. Negotiation is used to manage conflict and is the primary give-and-take process by which people try to reach an agreement~\cite{fisher2011getting,lewicki2011essentials}. Research on negotiation has been conducted for almost 60 years in the field of psychology, political science, and communication. \trackIZ{It has evolved over the past decades from exploring game theory~\cite{walton1991behavioral}, behavior decisions driven by the cognitive revolution in psychology~\cite{bazerman1993negotiating}, to cultural differences in the 2000s~\cite{bazerman2000negotiation}.}\noteIZ{Not clear -- please rephrase}
Negotiation research is now forced to confront the implications of human/AI collaborations 
given recent advancements in machine learning~\cite{sycara2010agent}.
%(Bazerman et al., 2000; Ouali, Sabouret & Rich, 2017). 
Combining insights from social scientists and data scientists will be fruitful in 
\trackIZ{maximizing expectations and outcomes during negotiation processes.}\noteIZ{Huh?}

%%Negotiation is a process by which two or more parties attempt to resolve their opposing interests.
\lizhen{Is it possible to have a definition for distributive and integrative respectively?}
A negotiation strategy can be \textit{distributive}, such as bargaining~\cite{fershtman1990importance},\noteIZ{Why doesn't bargaining maximize one's interest?} 
or \textit{integrative}, such as maximizing unilateral interests~\cite{bazerman1993negotiating}. Both 
types of strategies are used in various situations, \eg\ informal, peer to peer, organizational and 
diplomatic country to country settings. 
%%The implications for enhancing outcomes are thus large and important to understand. 
Research from psychology demonstrates that the negotiation process can be affected by psychological 
factors, such as personality~\cite{sharma2013role}, relationships~\cite{olekalns2003testing}, 
social status~\cite{blader2012differentiating} and cultural background~\cite{leung2011within}.  

==> 9_related_work.tex <==
\section{Related Work}

other relevant survey work on dialogue systems.
